All-relevant feature selection using multidimensional filters with exhaustive search

This paper describes a method for identification of the informative variables in the information system with discrete decision variables. It is targeted specifically towards discovery of the variables that are non-informative when considered alone, but are informative when the synergistic interactions between multiple variables are considered. To this end, the mutual entropy of all possible k-tuples of variables with decision variable is computed. Then, for each variable the maximal information gain due to interactions with other variables is obtained. For non-informative variables this quantity conforms to the well known statistical distributions. This allows for discerning truly informative variables from non-informative ones. For demonstration of the approach, the method is applied to several synthetic datasets that involve complex multidimensional interactions between variables. It is capable of identifying most important informative variables, even in the case when the dimensionality of the analysis is smaller than the true dimensionality of the problem. What is more, the high sensitivity of the algorithm allows for detection of the influence of nuisance variables on the response variable.

==> fs4_algorithm.tex <==
\section{The algorithm}

The theory described above leads to the algorithm of multivariate feature selection. It consists of the following steps:
\begin{itemize}
\item If the response variable and the explanatory variables are continuous, they should be discretized first.
\item For each $k$-tuple of variables $S^k$ the contingency table is built, that contains number of objects, for which the variables take on particular values. This step is the most expensive computationally, yet simple, so it can be performed using GPU.
\item For each variable $X\in S^k$ the conditional mutual information between the response variable $Y$ and $X$ given the rest of the $k$-tuple $S^{k-1}$ is calculated. Then, the associated $\chi^2$~$p$-value is calculated.
\item For each variable the minimum $p$-value over all the $k$-tuples is recorded as $p_{min}(X)$.
\begin{quote}
In the special case, when all the explanatory variables have the same number of categories (e.g. they are all the discretized continuous variables), the last two steps can be simplified. In this case the minimum $p$-value corresponds to the maximum value of $I(Y;X|S^{k-1})$. Instead of computing all the $p$-values, it is enough to record the maximum $I(Y;X|S^{k-1})$, then calculate the associated $p$-value once for a variable.
\end{quote}
\item Based on the statistics of $p_{min}$ over all the variables, the parameter $\gamma$ in Eq.~(\ref{expmin}) is estimated (see Appendix~\ref{statmax}).
\item The eventual $p$-value is calculated for each variable.
\item Bonferroni-Holm FWER method or Benjamini-Hochberg FDC method is used to decide, whether the variable should be selected as relevant.
\end{itemize}
